High-Stability Deformable Mirrors for Correcting Non-Axisymmetric Residual Aberrations in Thermal Compensation of Future Gravitational Wave Interferometers

In gravitational wave detectors, optical aberrations arise mainly from laser absorption in coatings and production process defects in the optics along the laser path. If left uncorrected, these optical path distortions drive the interferometer away from its optimal working point, degrading both stability and sensitivity. Future instruments such as the Einstein Telescope high-frequency detector will operate with unprecedented circulating power, further amplifying the aberration budget. In the current detectors Advanced Virgo and Advanced LIGO, the axisymmetric distortions are corrected using thermal actuators and CO2 laser projectors, however, non-axisymmetric wavefront distortions remain unmitigated. Deformable mirrors are investigated as a flexible solution for mitigating such defects: by shaping the CO2 beam phase upon reflection, they can imprint the required asymmetric intensity pattern on the lensing optics without introducing frequency dependent noise. The target phase map is computed via a modified Gerchberg-Saxton algorithm. We present simulations of this projection strategy and experimental validation demonstrating consistent reproduction of the desired intensity patterns.

==> old_introduction.tex <==
\section{Introduction}
The level of attainable accuracy and sensitivity in precision measurement schemes based on interferometric techniques strictly depends on the dark fringe contrast, that is, any residual light in the recombined pattern results in spoiling the shot-noise-limited sensitivity. This is particularly relevant for gravitational wave interferometric detectors operated at high input optical power as Advanced Virgo~\cite{} and Advanced LIGO~\cite{}. When the wavefront and amplitude distribution of the fields of the recombined laser beams at the output port are not perfectly matched, excess light content contaminates the dark fringe. The differential content of optical aberration is related to wavefront distortions that are different in the two interferometer arms. However, even aberrations in the common path can severely affect the detector operation at the level of controllability. This happens indeed in power-recycled interferometers, where the power recycling cavity resonance is controlled by sideband signal extraction techniques~\cite{?}. The field sidebands resonance condition is severely spoiled by wavefront distortion due to defects in the optics or thermal lensing caused by optical power absorption (mainly driven by optical coatings)~\cite{?}. 

The problem can be stated as follows: any deviation from the detector’s optical ideality must be kept below a well-defined requirement in order to prevent both a loss of controllability and a degradation of sensitivity. Strategies to achieve this result usually encompass three steps: first the list of requirements is identified and evaluated by means of careful simulation of the detector behavior versus wavefront distortions. Then, a system for sensing and control is developed and tested. Finally, the system is integrated in the detector layout and commissioned. Here we focus on the techniques adopted to actively control the budget of wavefront distortions. We shall consider the amount of wavefront aberration gathered by the beam when it passes through one of the input mirrors of the interferometer arm cavities and is reflected by the mirror coating back through the bulk and toward the recycling cavity. This approach does not cover all possible sources of aberration in a detector, but it allows to clearly and comprehensively frame the class of problems this article addresses. The solution described here is, however, capable of considerable versatility, which greatly expands its field of applicability.

First order aberrations are the main drivers of detector instability. An induced tilt or a constant optical path added to the wavefront can be easily compensated using mirror displacement or the angular controls of the interferometer. As a consequence, the dominant contribution to the wavefront uncompensated aberration is usually the spherical component, corresponding to a quadratic term in the optical path length
% Mettere da qui l'acronimo OPL?
distortion. According to this consideration, the first-generation thermal compensation strategies for Advanced Virgo were aimed to correct spherical aberration (also referred to as thermal defocus) or higher (even) order axisymmetric terms. An important case is the optical path length change due to the absorption of the optical power of the circulating laser beam on the mirror surface, which is strictly axisymmetric and can be developed in even order aberration terms. The latter is currently compensated using a compensation plate in front of the mirror on the recycling cavity side, shined with a CO$_2$ laser beam (totally absorbed at the surface) properly shaped to produce a complementary divergent aspheric lens via thermo-optic and thermo-elastic effects. The optimal heating profile is obtained numerically, while it is constructed experimentally by means of the sum of two annular profiles produced using a double-axicon optical system (DAS~\cite{?}).

Despite its noticeable success in controlling thermal effects in the marginally stable recycling cavity of Advanced Virgo during O3 and O4, the sole DAS-based approach could not be pursued in future detector upgrades driven by laser power enhancement. This is basically due to the following reasons:
\begin{itemize}
    \item The power distribution of the obtained DAS rings is usually not regular due to CO$_2$ laser bad modes, imperfections in the optics of the shaping system, angle of incidence. Such irregularity is responsible for an asymmetric uncompensated optical path length (OPL) distortion that can easily surpass the requirements. To give an idea, the residual RMS OPL distortion in the input mirror due to typical DAS imperfections reaches up to $20nm$ for $80W$ input power, to be compared with a requirement of $2nm$ RMS. An improved layout with stable recycling cavities would partially mitigate the issue, although it would reappear with a further increase in input power\footnote{The causes of the irregularity in the DAS profile can be addressed with properly designed upgrades such as mode cleaner cavities, improved optical design, optimized centering, at the cost of considerably complicating the system and its management, with the further disadvantage of making it less versatile.}.
    \item Inhomogeneous, asymmetrical defects are expected to be present in the optics. Point-dependent diffusion or refraction index are present in the mirror bulk, while dielectric coatings exhibit spatial variability of absorption that could give rise to an asymmetric thermal lens. Though very low, these inhomogeneities set a budget of asymmetric, unavoidable OPL distortion likely limiting the attainment of high circulating power in future interferometers.
    \item Asymmetric residual OPL deformation can be produced by the action of other thermal actuators that are not directly related to the thermal lensing expected in the input mirrors. These actuators belong to two categories: those responsible for correcting the surface profile of the mirrors (ring heaters, thermal radiators) and those specifically developed to face unexpected problems.
\end{itemize}
The relevance of these reasons is such that the need for a corrector to address non-axisymmetric wavefront deformations were considered since the first generation of detectors, and various solutions were proposed. A fast CO$_2$ beam-based scanning system was originally proposed by Lorentz in his PhD thesis~\cite{?}, to produce an arbitrary heating pattern over a matrix of points. The main disadvantage of this approach is the displacement/lensing noise coupling to the detector sensitivity due to the point-by-point and scan-by-scan frequencies~\cite{?}.

An ideal static corrector, able to heat the compensation plate with an arbitrary and constant asymmetric pattern, would produce 
a stable asymmetric thermal lens optimized to compensate for residual non-axisymmetric wavefront deformations in the recycling cavity\footnote{Notice that in practice the required thermal lens should be determined through a direct measurement of the wavefront aberration budget, usually provided by local Hartmann wavefront sensors. The discussion about the practical determination of the optimal heating pattern is not in the scope of this paper.}. A real static actuator can be obtained, with a set of technical limitations, by shaping a CO$_2$ laser beam with a phase or intensity correction on an object plane. 
Intensity correction can be produced using binary masks or liquid crystal devices (LCD). While static masks lack the requisite versatility, LCD are typically limited to low power applications and are therefore not suitable for high power CO$_2$ beams. 
Therefore, the most effective and robust approach identified by the authors consists in using phase actuators such as deformable mirrors 
% Inserire qui l'acronimo DM?
. Deformable mirror devices represent a mature technology capable of high power operation and long term stability. Since their use is characteristic of astronomic imaging, most of their features are optimized for that kind of application.  Basic features include:
\begin{itemize}
    \item Mirror aperture and coating absorption at CO$_2$ wavelength ($10.6\mu m$). To avoid over-heating of the mirror membrane, the higher is the absorption the larger must be the aperture. Typical apertures are in the range of few $cm$.
    \item The mirror membrane is shaped by an array of actuators placed on the rear face. Actuators are usually very fast but not particularly stable, since their use in astronomy always includes a loop control. The most diffused actuator technologies are based on magnetic coils, electrostatic force  or piezoelectric crystals. 
    \item The actuator number and arrangement set a limit to the higher spatial frequency deformation that can be obtained. Usually an estimation based on the inverse of the actuator pitch $p$ is a reasonable estimate of the maximum frequency:
    \begin{equation}
        f_{max}\sim \frac{1}{2p}
    \end{equation}
    \item The maximum surface displacement range due to a single actuator with all other actuators held at their bias (stroke). The stroke must be at least of the order of fractions of the laser beam wavelength to have a compact beam shaping system.
\end{itemize}
